Saying Hello World with UML-RSDS - A Solution to the 2011 Instructive Case

In this paper we apply the UML-RSDS notation and tools to the "Hello World" case studies and explain the underlying development process for this model transformation approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{325}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.26}{10.4204/EPTCS.74.26}}

